Semantic Relational Object Tracking

This paper addresses the topic of semantic world modeling by conjoining probabilistic reasoning and object anchoring. The proposed approach uses a so-called bottom-up object anchoring method that relies on the rich continuous data from perceptual sensor data. A novel anchoring matching function method learns to maintain object entities in space and time and is validated using a large set of trained humanly annotated ground truth data of real-world objects. For more complex scenarios, a high-level probabilistic object tracker has been integrated with the anchoring framework and handles the tracking of occluded objects via reasoning about the state of unobserved objects. We demonstrate the performance of our integrated approach through scenarios such as the shell game scenario, where we illustrate how anchored objects are retained by preserving relations through probabilistic reasoning.

==> tmp.tex <==
% --------------------------------

% Introduction
In order to have an efficient bottom-up anchoring approach, which is able to maintain anchors in real-time, it is essential to have an anchor matching procedure that is further able to handle the constant stream of perceived objects and accurately anchor perceived objects. However, erroneous readings will undoubtable be present in the the same stream of perceptual data, and consequently, also in the anchoring procedure. It is, therefore, also of importance to couple the the anchoring procedure with an appropriate data association procedure in order to compensate for error readings that emerge from the stream of perceptual data. 

% Background (removed parts)

%Moreover, it is also essential for the anchoring system to both recognize previously observed objects and detect (or anchor) new previously unknown objects. As a result, an anchoring matching procedure can not exclusively rely on single features.
%It is also essential to both recognize previously observed objects and detect (or anchor) new previously unknown objects. As a result, an anchoring matching procedure can not exclusively rely on single features.
%The types of features, or anchor attributes, used for the work in this paper is further presented in Section~\ref{section:method}. 
%The largest concern regarding matching of features in the context of bottom-up perceptual anchoring is that anchoring is concerned with real physical objects. It is, therefore, also essential to both recognize previously observed objects and detect (or anchor) new previously unknown objects. As a result, an anchoring matching procedure can not exclusively rely on single features.
 
%-- However, in previously reported work on perceptual anchoring, the problem of matching the features of anchors, and consequently also matching of anchors, have mostly been simplified or left out entirely \todo{Need a slightly better motivation, e.g. all previously reported work on perceptual anchoring have simplified the matching problem through the use of symbolic values, etc. }. However, moving the procedure of matching anchors down to the perceptual level will, undoutable, also introduce another level of complexity. Considering open world scenarios, this complexity will no doutably become an issue. In this paper, we will address this issue and present an evaluation that addresses the problem of matching features at scale in the context of perceptual anchoring. The largest concern regarding matching of features in the context of perceptual anchoring is that anchoring is concerned with real physical objects. It is, therefore, also essential to both recognize previously observed objects and detect (or anchor) new previously unknown objects. As a result, an anchoring matching procedure can not exclusively rely on single (or simplified) features. The types of features, or anchor attributes, used for the work in this paper is further presented in Section~\ref{section:method}.

%++ However, in previously reported work on perceptual anchoring, the problem of matching the features of anchors, and consequently also matching of anchors, have mostly been simplified through the use of symbolic values, or left out entirely. In case of a simplified approach through matching based on symbolic values, such approach will inevitable also introduce ambiguous results (since the symbolic system can only consist of a discrete number of symbols). Hence, the procedure of creating and maintaining anchors, on the symbolic level, must either be handled strictly probabilistically, as in the case of \citep{elfring.et.al-2013}, or through the use of additional knowledge through the use of a reasoning systems, as in the case of \cite{daoutis.et.al-2012}. However, both the works presented by \citep{elfring.et.al-2013} and \cite{daoutis.et.al-2012} utilized a conceptual space, exemplified in Figure~\ref{}, in order to establish the predicate grounding relation between measured attribute values and predicate symbols, and where the mapped predicate symbols were, subsequently, used for the purpose of determine if a perceived object has previously been anchored or not. 

%The intuition behind this work is that; moving from measurable attribute values to predicate symbols, as exemplified in Figure~\ref{}, and basing the anchoring matching procedure on symbolic values, will consequently also result in an tremendous loss of information (since measurable attribute values are continues). However, moving the procedure of matching anchors down to the perceptual level will, undoubtable, also introduce another level of complexity. Concidering open world scenarios, this complexity will no doubtably become an issue. 

% Method
With the re-introduction of the track functionality, we further need to approach the issues of how to compensate for falsely acquired (or re-acquired) anchors. Hence, we have introduced an additional anchoring procedure for merging a falsely acquired anchor with its original anchor counterpart - the anchor that in a prior time-step, $t-1$, was not correctly maintained through the re-acquired functionality. This procedure takes the the perceptual and symbolic properties of an falsely acquired anchor $\alpha_a$ and update the perceptual and symbolic properties of the associated anchor $\alpha_b$, such that $\alpha_{b=a}$ is defined at time $t$. The falsely acquired anchor $\alpha_a$ is, subsequently, deleted from the anchor-space. 

% Results


% Conclusions
In this paper, we have presented how we are able to improve the overall anchoring process by introducing an post-anchoring data association procedure, with the purpose of predicting the probability of false-negatively acquired anchors, and subsequently, compensate for such falsely acquired anchors. We have further presented an novel approach for learning how to determine, in the first place, if an perceived object has previously been perceived or not. Through the presented results, we have shown that our object anchoring approach is able to accurately anchoring objects and maintaining consistent representations of object with an accuracy of $XX\%$. 

% --------------------------------

